CNC-Net: Self-Supervised Learning for CNC Machining Operations

CNC manufacturing is a process that employs computer numerical control (CNC) machines to govern the movements of various industrial tools and machinery, encompassing equipment ranging from grinders and lathes to mills and CNC routers. However, the reliance on manual CNC programming has become a bottleneck, and the requirement for expert knowledge can result in significant costs. Therefore, we introduce a pioneering approach named CNC-Net, representing the use of deep neural networks (DNNs) to simulate CNC machines and grasp intricate operations when supplied with raw materials. CNC-Net constitutes a self-supervised framework that exclusively takes an input 3D model and subsequently generates the essential operation parameters required by the CNC machine to construct the object. Our method has the potential to transformative automation in manufacturing by offering a cost-effective alternative to the high costs of manual CNC programming while maintaining exceptional precision in 3D object production. Our experiments underscore the effectiveness of our CNC-Net in constructing the desired 3D objects through the utilization of CNC operations. Notably, it excels in preserving finer local details, exhibiting a marked enhancement in precision compared to the state-of-the-art 3D CAD reconstruction approaches.

==> sections/figures/ablation_steps.tex <==
\renewcommand\thesubfigure{}

\begin{figure}
     \centering
     %%%%%%%%%%%%%%%%%%%%%%%%%%%  %%%%%%%%%%%%%%%%%%%%%%%%%%
     \begin{subfigure}[b]{0.06\textwidth}
        \centering
        \includegraphics[width=\textwidth]{example-image-a}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.06\textwidth}
        \centering
        \includegraphics[width=\textwidth]{example-image-a}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.06\textwidth}
        \centering
        \includegraphics[width=\textwidth]{example-image-a}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.06\textwidth}
        \centering
        \includegraphics[width=\textwidth]{example-image-a}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.06\textwidth}
        \centering
        \includegraphics[width=\textwidth]{example-image-a}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.06\textwidth}
        \centering
        \includegraphics[width=\textwidth]{example-image-a}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.06\textwidth}
        \centering
        \includegraphics[width=\textwidth]{example-image-a}
     \end{subfigure}

     %%%%%%%%%%%%%%%%%%%%%%%%%%%  %%%%%%%%%%%%%%%%%%%%%%%%%%
     \begin{subfigure}[b]{0.06\textwidth}
        \centering
        \includegraphics[width=\textwidth]{example-image-a}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.06\textwidth}
        \centering
        \includegraphics[width=\textwidth]{example-image-a}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.06\textwidth}
        \centering
        \includegraphics[width=\textwidth]{example-image-a}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.06\textwidth}
        \centering
        \includegraphics[width=\textwidth]{example-image-a}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.06\textwidth}
        \centering
        \includegraphics[width=\textwidth]{example-image-a}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.06\textwidth}
        \centering
        \includegraphics[width=\textwidth]{example-image-a}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.06\textwidth}
        \centering
        \includegraphics[width=\textwidth]{example-image-a}
     \end{subfigure}

     %%%%%%%%%%%%%%%%%%%%%%%%%%%  %%%%%%%%%%%%%%%%%%%%%%%%%%
     \begin{subfigure}[b]{0.06\textwidth}
        \centering
        \includegraphics[width=\textwidth]{example-image-a}
        \caption*{Input}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.06\textwidth}
        \centering
        \includegraphics[width=\textwidth]{example-image-a}
        \caption*{Step~0}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.06\textwidth}
        \centering
        \includegraphics[width=\textwidth]{example-image-a}
        \caption*{Step~10}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.06\textwidth}
        \centering
        \includegraphics[width=\textwidth]{example-image-a}
        \caption*{Step~20}
     \end{subfigure}
    \hfill
     \begin{subfigure}[b]{0.06\textwidth}
        \centering
        \includegraphics[width=\textwidth]{example-image-a}
        \caption*{Step~50}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.06\textwidth}
        \centering
        \includegraphics[width=\textwidth]{example-image-a}
        \caption*{Step~last}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.06\textwidth}
        \centering
        \includegraphics[width=\textwidth]{example-image-a}
        \caption*{Target}
     \end{subfigure}

        \caption{
        % 
        \textbf{Intermediate results on ABC~\cite{Abc} dataset.} 
        %
        }
        \label{fig:ablation_steps}
\end{figure}     


==> sections/tables/ablation_steps.tex <==
\begin{table}[t]
\small
    \begin{center}
        \setlength\tabcolsep{3pt}
        \begin{tabular}{lccc}
            \hline
            N & min & avg & max\\
            \hline
            ABC & 000 & 000 & 000 \\
            ShapeNet & 000 & 000 & 000\\
            \hline
        \end{tabular}
    \end{center}
    
    \caption{
        \textbf{Ablation study on the effect of losses.} 
        %
    }
    \label{tab:ablation_steps}
    \vspace{2mm}
\end{table}


==> sections/tables/vs_expert.tex <==
\begin{table}[t]
\small
    \begin{center}
        \setlength\tabcolsep{3pt}
        \begin{tabular}{lcccccccc}
            \hline
            Method & CD$\downarrow$ & ECD$\downarrow$ & CN$\uparrow$ & LFD$\downarrow$ & N$\downarrow$ & P$\downarrow$ & T$\downarrow$ & R$\downarrow$  \\
            \hline
            $\mathcal{L}^{\text{rec}}$ & 000 & 000 & 000 & 000 & 000 & 000 & 000 & 000  \\
             Person 1 & 000 & 000 & 000 & 000 & 000 & 000 & 000 & 000  \\
             Person 2 & 000 & 000 & 000 & 000 & 000 & 000 & 000 & 000  \\
             CAD 1 & 000 & 000 & 000 & 000 & 000 & 000 & 000 & 000  \\
             CAD 2 & 000 & 000 & 000 & 000 & 000 & 000 & 000 & 000  \\
            \hline
            $\mathcal{L}^{\text{total}}$ & 000 & 000 & 000 & 000 & 000 & 000 & 000 & 000  \\
            \hline
        \end{tabular}
    \end{center}

    \caption{
        \textbf{Comparison with experts.} We compare our results in terms of accuracy and efficiency with two human expert labors and ...
        %
    }
    \label{tab:experts}
    \vspace{2mm}
\end{table}

